Verified Subtyping with Traits and Mixins

Traits allow decomposing programs into smaller parts and mixins are a form of composition that resemble multiple inheritance. Unfortunately, in the presence of traits, programming languages like Scala give up on subtyping relation between objects. In this paper, we present a method to check subtyping between objects based on entailment in separation logic. We implement our method as a domain specific language in Scala and apply it on the Scala standard library. We have verified that 67% of mixins used in the Scala standard library do indeed conform to subtyping between the traits that are used to build them.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{S.-W. Lin and L. Petrucci (Eds.): 2nd French Singaporean\\ Workshop on Formal Methods and Applications\\
EPTCS 156, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.156.8}{10.4204/EPTCS.156.8}}

